TREE: Tree Regularization for Efficient Execution

The rise of machine learning methods on heavily resource constrained devices requires not only the choice of a suitable model architecture for the target platform, but also the optimization of the chosen model with regard to execution time consumption for inference in order to optimally utilize the available resources. Random forests and decision trees are shown to be a suitable model for such a scenario, since they are not only heavily tunable towards the total model size, but also offer a high potential for optimizing their executions according to the underlying memory architecture. In addition to the straightforward strategy of enforcing shorter paths through decision trees and hence reducing the execution time for inference, hardware-aware implementations can optimize the execution time in an orthogonal manner. One particular hardware-aware optimization is to layout the memory of decision trees in such a way, that higher probably paths are less likely to be evicted from system caches. This works particularly well when splits within tree nodes are uneven and have a high probability to visit one of the child nodes. In this paper, we present a method to reduce path lengths by rewarding uneven probability distributions during the training of decision trees at the cost of a minimal accuracy degradation. Specifically, we regularize the impurity computation of the CART algorithm in order to favor not only low impurity, but also highly asymmetric distributions for the evaluation of split criteria and hence offer a high optimization potential for a memory architecture-aware implementation. We show that especially for binary classification data sets and data sets with many samples, this form of regularization can lead to an reduction of up to approximately four times in the execution time with a minimal accuracy degradation.

==> sections/sysmodel.tex <==
% \daniel{I believe this section now is irrelevant, as everything we probably need to explain in here was already mentioned.}


Caches in modern CPUs are managed by prefetching and replacing, where the hardware automatically decides which contents to flush from the cache when it runs out of space, e.g., based on an age-based replacement strategy.
Furthermore, the memory hardware detects patterns in the memory accesses from the application and speculatively prefetches the assumed next accessed contents to the cache. 

% \christian{Added part}
% An orthogonal possibility to improve the performance is to reduce the total model size by controlling the training process to only keep important paths. The reduced total volume leads to a reduced amount of cache replacement and therefore to an improvement of the execution time. In addition, this regularization of the training can be designed in a way, that not only important paths in terms of prediction accuracy are kept, but important paths in terms of cache optimization with the algorithm of Chen et~al. are kept. 
%This consequently leads to an orthogonal optimization of the cache optimization from Chen et~al., since the cache friendly handling of frequently accessed paths is kept, and cache replacement are reduced.

% Hence, regularization with a focus on uneven splits promises to deliver performance increase, which is orthogonal to the algorithm from Chen et~al.
% \christian{End added part}
% As mentioned before, hardware aware optimization requires asymmetric probability distribution, i.e. trees which have certain paths executed significantly more often than other paths. 
% Such paths then can be favored in the memory hierarchy, such that their access is usually faster than the access to other paths. 
% Since this imposes possibly also a slowdown of other paths, the benefit can only compensate the cost when the optimized path is accessed comparably often.

Our regularization approach conceptually
%introduces a concept for regularization of the training of random forests in order to penalize even splits, i.e. 
rewards highly uneven split decisions in the training process.
With such uneven splits in the decision trees, certain nodes are more often accessed than other nodes. 
Accounting for the cache replacement, 
%highly uneven splits in decision trees and hence
more frequent accesses to few tree nodes form a small, frequently accesses working set, which ideally align with typical age-based cache replacement strategies, e.g., the well-known Least Recently Used (LRU) strategy.

Accounting for the cache prefetching, cache-aware optimizations like those proposed in~\cite{chen2022efficient}, place frequently accessed paths sequentially in memory, in order to benefit prefetching for the probably next accessed nodes. Provoking uneven splits helps such algorithms to more clearly identify frequently accessed paths and provide an according sequential memory layout. Hence, our approach is orthogonal to such optimizations, since the cache-aware handling of frequently accessed paths is persisted, and cache replacement are also reduced. 

%Accounting for the cache prefetching, cache-aware optimizations like those proposed in~\cite{chen2022efficient}, place frequently accessed paths sequentially in memory, in order to benefit prefetching for the probably next accessed nodes.
%Provoking uneven splits helps such algorithms to more clearly identify frequently accessed paths and provide an according sequential memory layout.

% Therefore, our approach is orthogonal to the cache-aware optimizations like in~\cite{chen2022efficient}, which favor frequently used paths based on the given asymmetric probability distribution, since the cache friendly handling of frequently accessed paths is kept, and cache replacement are reduced.

%consequently leading to an orthogonal optimization to the cache-aware optimizations, which rely on asymmetric probability distribution. %i.e. trees which have certain paths executed significantly more often than other paths. 
% Such paths then can be favored in the memory hierarchy, such that their access is usually faster than the access to other paths. 
% Since this imposes possibly also a slowdown of other paths, the benefit can only compensate the cost when the optimized path is accessed comparably often.




%As shown in related works, such uneven splits effectively help to improve the execution time performance when a subsequent cache optimization of the forest is performed.



% \kuan{we didn't talk about what is the target system right?}
% With a target system with a few kB sized level~1 cache, the random forest rapidly exceeds the total size of the level 1 cache. 
% Since accesses to the level 1 cache are much faster, reducing the number of cache misses helps to improve the allover execution time.
%Keeping these nodes local in the level 1 cache is the ultimate goal of the optimization.



%which is protected from preemption by the data age based cache management.



%orthogonal possibility to improve the performance is to reduce the total model size by controlling the training process to only keep important paths. The reduced total volume leads to a reduced amount of cache replacement and therefore to an improvement of the execution time. In addition, this regularization of the training can be designed in a way, that not only important paths in terms of prediction accuracy are kept, but important paths in terms of cache optimization with the algorithm of Chen et~al. are kept. 
%This consequently leads to an orthogonal optimization of the cache optimization from Chen et~al., since the cache friendly handling of frequently accessed paths is kept, and cache replacement are reduced.


==> sections/tree-optimization.tex <==
Decision trees offer a great opportunity to improve performance of the inference.
It has been shown that rearranging the memory layout of the nodes can lead to a considerable reduction in execution time without any change in the logic tree model \cite{chen2022efficient}. 
Using an underlying probabilistic model of the tree, a memory layout is generated, in which data locality of the nodes is improved, leading to fewer cache-misses.


% \christian{Expand a bit:}
% Chen et~al. introduce an algorithmic way to utilize this probability distribution for cache optimization \cite{chen2022efficient}. 
% Utilizing the prefetching property of caches, the higher probable child ideally is already prefetched while accessing previous nodes, such that the higher probable case of executing the tree features less cache misses.
% Since the prefetching in caches detects linear ascending memory access patterns, Chen et~al. place high probable paths linearly in memory, such that they are hit by prefetching.
% The more asymmetric the probability distribution in single nodes is, the more often the cache optimized case occurs, and the less latency is caused overall.
% \christian{End of expamd}




